Mix and Match: Learning-free Controllable Text Generation using Energy Language Models

Recent work on controlled text generation has either required attribute-based fine-tuning of the base language model (LM), or has restricted the parameterization of the attribute discriminator to be compatible with the base autoregressive LM. In this work, we propose Mix and Match LM, a global score-based alternative for controllable text generation that combines arbitrary pre-trained black-box models for achieving the desired attributes in the generated text without involving any fine-tuning or structural assumptions about the black-box models. We interpret the task of controllable generation as drawing samples from an energy-based model whose energy values are a linear combination of scores from black-box models that are separately responsible for fluency, the control attribute, and faithfulness to any conditioning context. We use a Metropolis-Hastings sampling scheme to sample from this energy-based model using bidirectional context and global attribute features. We validate the effectiveness of our approach on various controlled generation and style-based text revision tasks by outperforming recently proposed methods that involve extra training, fine-tuning, or restrictive assumptions over the form of models.

==> body/intro.tex <==
\section{Introduction}
%\kg{start here...}
%\begin{SCfigure*}[][t]
 \begin{figure}
    \centering
     \includegraphics[width=0.95\textwidth]{figs/overview_fig_v2.pdf}
     \caption{Overview of Mix and Match LM. The Lego pieces show different experts that can be used to form the energy LM and help control different features in the generated text. The right side shows the $i$th step in the the Gibbs sampling chain, where a proposal is made by the MLM, and then it is accepted/rejected based on the energy score.}
     \label{fig:mmlm}
    % \begin{subfigure}{0.28\textwidth}
    %  \includegraphics[width=\linewidth]{figs/mnist_dpsgd_15.png}
    %  \caption{MNIST DPSGD for $\varepsilon=15$}
    %  \label{fig:blogs-2dom-unc}
    % \end{subfigure}
    \vspace{-2ex}
\end{figure}
 %\end{SCfigure*}
 
Transformer-based language models trained on massive amounts of natural language data found on the internet have demonstrated exceptional ability to learn useful representations of sentences for downstream natural language processing tasks. Autoregressive models like GPT-3 are commonly used to \emph{generate} high quality natural language text as well. However, effective methods for generating well-formed sequences that satisfy a desired global control attribute (e.g., sentiment, formality, etc.) represent an active area of research. If successful, effective controlled generation techniques might help mitigate bias and prevent generation of hate speech and toxic language~\cite{fudge,xudetoxifying,gehman2020realtoxicityprompts}.

Much of the prior work on controlled generation has focused on autoregressive models like GPT-2 and has involved fine-tuning of these large models on target attributes~\cite{fudge,gedi}, or training entirely separate probabilistic generative models for the target attributes~\cite{he2020}, or training specialized attribute models with a restricted structure to heuristically generate attribute-sensitive sequences~\cite{pplm}. 
Our approach instead focuses on drawing samples from a test-time combination of pretrained blackbox experts that each score a desired property of output text -- for example, fluency, attribute sensitivity, or faithfulness to the context. Specifically, we view the product of these blackbox experts as a probabilistic energy model~\cite{poe} -- i.e., a non-autoregressive, globally normalized language model -- and then sample (without further training or fine-tuning) using a specialized Gibbs sampler with a Metropolis-Hastings correction step~\cite{MH}.
% Our approach instead focuses on a non-autoregressive setup to draw samples based on global features from a probabilistic model that is defined as a product of expert blackboxes energy model~\cite{poe}, with each blackbox being responsible for a salient aspect for generation like fluency, attribute sensitivity, faithfulness to the context etc.

Our full framework, which we entitle Mix and Match LM (depicted in Figure~\ref{fig:mmlm}), enables generation of high-quality attribute-controlled samples by mixing and matching blackbox models like off-the-shelf pretrained attribute-sensitive discriminators (e.g., sentiment classifiers), large bidirectional pretrained language models like BERT~\cite{bert}, and other modules specializing in capturing desirable features pertaining to faithfulness to any additional context, like hamming distance, BertScore distance~\cite{bertscore}, or Bleurt~\cite{bleurt} based distance between the sample and the conditioning context. 
% We define an energy-based probabilistic sequence model whose underlying energy values are a linear combination of scores from these blackbox modules i.e. a globally normalized mixture of experts model.
% We interpret the task of controlled generation or controlled revision as generating samples from this energy-based sequence model.
We generate samples from the energy language model assembled from these component experts
% model based upon rich bidirectional context and global features 
by using the recently proposed Gibbs-Metropolis-Hastings scheme~\cite{MH} for sampling from energy models using a masked language model as a proposal distribution. In this scheme, an expressive bidirectional language model like BERT is used to make a proposal at each transition step in the Gibbs chain to jump to a sequence $\mathbf{\bar{x}}$ from the current sequence $\mathbf{x}$. This proposal's fitness is judged by the change in the energy language model's score, with the sampler accepting proposals with larger energy reductions at a higher rate. This approach yields high-quality diverse samples that respect the distribution induced by the product of expert blackbox models. 

We demonstrate the flexibility of our approach by performing a variety of controlled generation tasks, such as aspect-based text revision, style transfer, and attribute grounded generation. On all of these tasks, we compare our performance to existing approaches that involve additional fine-tuning of generation or attribute based models, or impose restrictions on the parametrization of specific components. We observe that our approach, which does not require any gradient optimization and is able to combine arbitrary heterogeneous blackbox models, outperforms recent controllable generation and style transfer models on a variety of tasks according to various automated metrics of fluency, quality, and control, as well as human evaluations.
%\kg{end here...}

%With the advent of large transformer-based models trained on huge amounts of data, language modeling and generation have seen great progress, generating human-like sentences.
%
%However, since these models are trained on web-scraped, unscrubbed data, the text generated by them (sampled from $P(X)$) could contain bias, hate speech, toxicity, or it could just have style or tone that is different from what is desired for downstream tasks. 
%
%To address these drawbacks, controlled generation~\cite{some} and style transfer techniques attempt at generating text with a given attribute ($P(X|a)$), or revising/re-generating given text ($P(X|p,a)$). 
%

%

%Some prior work do this by retraining or finetuning  the large model on domain-specific data~\cite{}, or by modifying the architecture of the pre-trained model~\cite{}. Same goes for style transfer, where large generative models are trained with parallel~\cite{} or unparallel~\cite{} datasets for transfering style between to domains. 
%
%Li et al. (2018) demonstrate the efficacy of a simple approach based on replacing attribute related n-grams with n-grams correspond- ing to the desired attribute based on a conditional generative model.
%
%However, training (or fine-tuning) a new LM for each attribute or introducing a new model architecture is inefficient and incurs huge training and manual overheads.
%
%To alleviate these overheads, recent work use attribute discriminators to guide the generation process. 
%
%Plug and Play LM (Dathathri et al., 2020, PPLM) uses  discriminators learned from the LM's top-level hidden layer to modify the LM's states toward increasing probability of the desired attribute via gradient ascent. This applies up to 10 updates to the generating LM’s latent states per time step using gradients from a discriminator,  making it many times slower than generating from the LM directly.
%
%GeDi and Fudge take similar, approaches and guide generation from LM using specially trained generative and future discriminators, respectively. 
%
%None of these works however, are completely training free, and they all need some type of ad-hoc discriminator or training process, suited for the given framework.


%We proposed mix and match LM, a framework that can take out of the box, pre-trained discriminators, mix and match them with other heuristics coming from different modules. These heuristics could be  hamming distance (for preserving sentence structure), or BertScore (for preserving sentence meaning) or even agency score (for removing gender-related agency bias) and combine them all at test-time seamlessly, without any training, to create an energy model. We then sample directly from this energy, using Metropolis-Hastings gibbs sampler~\cite{kartik}. 
%
%???
%

%Our approach can be readily applied to any controlled generation task, such as attribute grounded generation or style transfer. We evaluate our model on two style transfer tasks (sentiment and formality transfer), where we compare our results with that of~\cite{he2020}, a probabilistic VAE-based generative model, agency bias removal  where we compare with PowerTransformer~\cite{}. We also experiment with sentiment controlled prompted generation and compare our results with~\cite{pplm}. 


%The Transformer architecture (Vaswani et al., 2017) has enabled large-scale language models (LMs) trained on a huge amount of data (Radford et al., 2019; Dai et al., 2019b; Radford et al., 2018b) to greatly improve the state-of-the-art on natural language processing tasks. These models are used to extract contextualized word embeddings for transfer learning purposes (Devlin et al., 2019) and as natural language generators. The latter can leverage large amounts of unannotated data and a simple log-likelihood training objective. However, once such models are trained, controlling attributes of generated text becomes difficult without modifying the model architecture to allow for extra input attributes or fine-tuning with attribute-specific data (Keskar et al., 2019; Ziegler et al., 2019).

%Optimization is performed ex post facto in the activation space, therefore no re-training or fine- tuning is needed. Control is fine-grained, with a strength parameter determining how strong the attribute influence should be; a strength of 0 fully recovers the original model p(x). This design allows vast flexibility: users can combine a state-of-the-art generative model, which may be large and difficult to train, with any number of attribute controllers. 






%We run experiments on three controlled text generation tasks — couplet completion in poetry, topic control in language generation, and formal- ity change in machine translation — showing our method’s broad applicability. Additionally, we demonstrate the modularity of FUDGE by com- posing multiple attribute constraints in both the couplet and topic control tasks.


==> body/related_work.tex <==
\section{Related Work}
%A large body of prior work has focused on controlled generation with massive autoregressive language models like GPT-2 and much of the work on style transfer shares similar goals of flexible attribute based generation. 
%techniques attempt at generating text with a given attribute ($P(X|a)$), or revising/re-generating given text ($P(X|p,a)$). 
%A large body of prior work on controlled generation and style transfer focuses on flexible attribute-base generation. Some 
A large body of work has approached the porblem of controlled generation via either training \cite{prabhumoye-etal-2020-exploring, he2020, lample2018phrase,shen2017style,Krishna2020ReformulatingUS, reif2021recipe, ficler-goldberg-2017-controlling, khalifa2021a} domain-conditioned neural language models or finetuning/modifying an underlying large pretrained base model for generation on domain-specific data~\cite{ziegler2019fine, keskar2019ctrl,mai-etal-2020-plug,gururangan-etal-2020-dont} for attribute sensitive generation which is computationally expensive and data intensive. 
%These methods not only add to the computational expense of training for controlled generation but crucially, also depend on the availability of and access to attribute sensitive language data which limits the scenarios in which these approaches can be used.  
%Common approaches for flexible attribute-based generation range from retraining or fine-tuning a large underlying base model for generation on domain-specific data~\cite{ziegler2019fine}, to modifying the architecture of the large pre-trained model~\cite{keskar2019ctrl}. Several style transfer approaches hinge on training large generative models with  non-parallel~\cite{he2020,lample2018phrase,shen2017style,Krishna2020ReformulatingUS,reif2021recipe} data across the domains of interest. 
%
%Li et al.\cite{}  (2018) demonstrate the efficacy of a simple approach based on replacing attribute related n-grams with n-grams correspond- ing to the desired attribute based on a conditional generative model. \kg{what is this? non-neural? where dsoes it go in the discussion}
%
%However, training (or fine-tuning) a new LM for each attribute or introducing a new model architecture is inefficient and incurs huge training and manual overheads.
%

Our work eschews training and focuses on generation-time control from pretrained modules. Recent work in this space has used attribute discriminators \cite{pplm, gedi, fudge, holtzman-etal-2018-learning} to steer the generation \nocite{gu-etal-2017-trainable} from a large autoregressive language model. 
%
Plug-and-Play LM~\cite{pplm} uses  discriminators learned from the LM's top-level hidden layer to modify the LM's states toward increasing probability of the desired attribute via gradient ascent at each step. This restricts the parametrization of the discriminator and also requires access to multiple gradients from the discriminator multiple times per generated sentence, making this approach fairly expensive and restrictive.
%
GeDi~\cite{gedi} and FUDGE~\cite{fudge} take similar approaches and guide generation from an underlying autoregressive LM by training and using step-wise attribute-sensitive discriminators that decide whether the desired attribute is likely to be satisfied by the current generation path. GeDi trains class-conditional language models for these discriminators and hence additionally relies on access to attribute sensitive language data. DExperts~\cite{liu-etal-2021-dexperts} is another decoding-time controllable generation approach which modifies the stepwise softmax logits of an autoregressive pretrained LM with softmax logits of separately trained domain-specific \emph{expert} autoregressive language models. 
%
These approaches in addition to requiring some kind of optimization like training of auxilliary language models, or step-wise discriminators on partial autoregressive outputs, also rely on heuristics to manipulate the local softmax distributions of autoregressive models and do not enjoy the benefits of incorporating global features into the generation mechanism in a simple probabilistic manner.
In contrast, following the findings related to implicit energy-based models trained via non-probabilistic objectives \cite{grathwohl2019your, MH}, our energy-based formulation is not only optimization-free, but also fully modular and able to easily incorporate global features, allowing for heterogenous blackbox experts to be combined with each other.%and affect the non-autoregressive generation directly.
%None of these works however, are completely training free, and they all need some type of ad-hoc discriminator or training process, suited for the given framework.

%We divide the related work into two  groups, the prior work on controlled generation, and the work on style transfer. We expand each group below. 
%\paragraph{Controlled generation.}
%\paragraph{Style Transfer}

==> tables/fudge.tex <==
%  \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
\begin{tabular}{@{}cRccccccc@{}}
	\toprule
	%
	& {Method} & {Topic-score} & {Grammaticality} &{GPT-2 PPL}&{Div-Unig}	& {Div-Bi} & {Div-Tri} &{Human Preference(\%)} \\

% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
 

    \multirow{2}{*}{\STAB{}} & 
    %%%%%%%%%%&&&&&&&\\
    {FUDGE}	    &	1.45  & 0.61 &	{104.8}&  0.54&0.86&0.87& 37.5	\\
    %%%%%%%%%%&&&&&&&\\
    &\textbf{M\&M LM} (Ours) & 1.21 &0.74	& 110.2&	0.57&0.89&0.88& 62.5	\\
    %%%%%%%%%&&&&&&&\\

    %%%%%%%%%%&&&&&&&\\
	%%%%%%%%%
	\bottomrule
\end{tabular}


==> tables/pplm_sentiment.tex <==
%  \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
\begin{tabular}{@{}c@{\hskip 2mm}lSSSS@{}}
	\toprule
	%
	 &{Method} & {GPT-2} & {MLM} & {Int. Clsf.} & {Ext. Clsf.} \\

% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
     \multirow{3}{*}{\STAB{PPLM}} & 
    Length 12  &113.1& -137.1&71.9&58.03\\
    &Length 20 &61.1& -237.1&74.46&57.67\\
    &Length 50 &29.0&  -606.1&73.57&60.71\\
    %%%%%%%%%&&&&&&&\\
    \midrule[0.1pt]
 
    \multirow{3}{*}{\STAB{Ours}} & 
    Length 12  &264.1& -160.4&94.28&65.12\\
    &Length 20 &167.2&  -271.0&96.25&65.91\\
    &Length 50 &122.3& -692.3&93.8&68.57\\


    %%%%%%%%%%&&&&&&&\\
	%%%%%%%%%
	\bottomrule
\end{tabular}

